An Empirical Study on Robustness to Spurious Correlations using Pre-trained Language Models

Recent work has shown that pre-trained language models such as BERT improve robustness to spurious correlations in the dataset. Intrigued by these results, we find that the key to their success is generalization from a small amount of counterexamples where the spurious correlations do not hold. When such minority examples are scarce, pre-trained models perform as poorly as models trained from scratch. In the case of extreme minority, we propose to use multi-task learning (MTL) to improve generalization. Our experiments on natural language inference and paraphrase identification show that MTL with the right auxiliary tasks significantly improves performance on challenging examples without hurting the in-distribution performance. Further, we show that the gain from MTL mainly comes from improved generalization from the minority examples. Our results highlight the importance of data diversity for overcoming spurious correlations.

==> appendices.tex <==
\section{Appendices}

Table~\ref{tab:pretrainedBert_more} and Table~\ref{tab:finalnli_more} show some experiment results on the three subsets of HANS.
Table~\ref{tab:pretrainedBert_more} shows the non-pretrained model and pretraind model results. And Table~\ref{tab:pretrainedBert_more} shows the model performance when adding the auxiliary datasets. 

\begin{table*}[ht]
\footnotesize{
  \begin{center}
  \tabcolsep 2pt
    \begin{tabular}{cccc} 
    \toprule
       Model   & \textbf{HANS-O(\%)}   & \textbf{HANS-C(\%)} & \textbf{HANS-S(\%)}     \\
      \midrule
      \multicolumn{1}{l}{\textbf{Non-pretrained Models}} \\
      \rbert  & 49.9(.04) & 49.3(0.1) & 50.3(0.4) \\ \hline \hline
      \multicolumn{1}{l}{\textbf{Pretrained Models}} \\
      %BERT$_{base}$(4 epochs) & MNLI-en & 84.5  & -  & - & - & 58.3  \\
      %\small{\citet{clark-etal-2019-dont}} &  & 84.2  &- & -& -& 62.4 \\
      \bert   & 75.8(4.9) & 59.1(4.8) & 52.7(1.2) \\
      \bertl  & 88.6(1.6) & 66.4(0.8) & 59.0(1.6) \\
      %Openwebtext-BERT  & 83.7/0.4 & 88 & 49 & & 68.2 \\ 
      \roberta & 88.5(2.0) & 70.0(2.3) & 63.9(1.4)  \\
      \robertal & 96.7(2.2) & 71.2(1.0) & 63.5(3.4) \\
      %mBERT$_{base}$ & MNLI-en & 82.7 & 76.3 &- &- & 65.0 \\
      %mBERT$_{base}$ & + translate & 58.0 &- &- &- &52.5 \\
      \bottomrule
    \end{tabular}
  \caption{\label{tab:pretrainedBert_more}Performance on HANS lexical overlap (HANS-O), HANS constituent (HANS-C) dataset, HANS subsequence (HANS-S) dataset when fine-tuning different BERTs: \rbert, \bert, \bertl, \roberta, and \robertal.  \rbert is \bert model with random initialization. For all the models, we do early stopping on the MNLI dev set and shows the means and standard deviations with 5 runs with different random seeds. The numbers in the bracket are the standard deviations of the 5 runs.}
  \end{center}
  }
\end{table*}



\begin{table*}[t]
\footnotesize{
 \begin{center}
%\tabcolsep 2pt
\begin{tabular}{ccccc}
%\toprule
 Task Data - Aux Data & \textbf{HANS-O(\%)} & \textbf{HANS-C(\%)}  &  \textbf{HANS-S(\%)}\\ 
 %\cline{3-7}
 %\midrule
 %MNLI(other paper), - & &  &  &  & \\
 MNLI  -  & 75.8(4.9) & 59.1(4.8) & 52.7(1.2)\\ \hline
MNLI , ALL
      &  89.5(1.9) & 61.9(2.3) & 53.1(1.1)\\
  
      
    % & DA & 84.2 & 90.9 & 91 & 28 \\ \midrule
    
    -PAWS
      &82.6(2.7) & 58.2(5.2) & 53.1(1.7)\\
    -QQP
     &  80.1(3.7) & 58.1(5.2) & 51.4(0.6) \\ 
    -SNLI
     &85.4(1.0)  & 61.1(2.2) & 54.3(1.0) \\ 
     
     \hline
     MNLI, PAWS
     & 82.3(1.8) & 59.4(3.9) & 52.8(1.0)\\ \hline    
%MNLI , SNLI + PAWS + QQP, $\gamma=5$
%      & 83.6 & 90.3 &  & & \\
     \bottomrule
\end{tabular}
    \caption{\label{tab:finalnli_more}The NLI experiment results of \bert on HANS three subsets: lexical overlap (HANS-O), constituent (HANS-C) and subsequence (HANS-S) when adding different auxiliary dataset: SNLI, \pawsqqp, \pawswiki, HANS. ALL = SNLI + PAWS + QQP. The numbers in the bracket are the standard deviations of the 5 runs.}
    \end{center}
    }
\end{table*}


==> mtl_results.tex <==
\subsection{Results}
\label{sec:mtl-results}
\paragraph{MTL improves robust accuracy.}
Our main MTL results are shown in \reftab{mtl_results}.
MTL increases accuracies on the challenging datasets across tasks
without hurting the in-distribution performance,
especially when the minority examples in the target dataset is scarce (\eg \paws).
While prior work has shown limited success of MTL when tested on in-distribution data\citep{sogaard2016deep,hashimoto2017joint,raffel2019exploring},
our results demonstrate its value for out-of-distribution generalization. 

\begin{table}[ht]
\footnotesize{
    \centering
    \tabcolsep 4pt
    \begin{tabular}{llrrr}
    \toprule
        Model & Algo.  & \textbf{HANS-O}   & \textbf{HANS-C} & \textbf{HANS-S}     \\
      \midrule
        \bert   & STL  & 75.8 (4.9) & 59.1 (4.8) & 52.7 (1.2) \\
        \bert   & MTL  & 89.5 (1.9) & 61.9 (2.3) & 53.1 (1.1) \\
        \roberta & STL & 88.5 (2.0) & 70.0 (2.3) & 63.9 (1.4)  \\
        \roberta & MTL & 90.3 (1.2)  & 64.8 (3.1)  &63.5 (4.9)     \\
        \bottomrule
    \end{tabular}
    \caption{\label{tab:hans_category}
    MTL Results on different categories on \hans: \texttt{lexical overlap} (O), \texttt{constituent} (C), and \texttt{subsequence} (S).
    Both auxiliary data (MTL) and larger pre-training data (RoBERTa) improve accuracies mainly on \texttt{lexical overlap}.
    }
}
\end{table}

\begin{table}[ht]
%\footnotesize{
\begin{center}
\begin{tabular}{lrrr}
\toprule
  Removed   &  \textbf{MNLI-m} & \textbf{HANS} & $\Delta$ \\ 
 \midrule

None
     &  83.7 (0.3) & 68.2 (1.8) & - \\  %& 90.4(0.1) 
\midrule
\pawsall            
      & 83.5 (0.3) & 64.6 (3.5) & -3.6\\   %& 90.3(0.3) 
QQP                               %            
      & 83.2 (0.3) & 63.2 (3.7) & -5.0 \\ %& 89.9(0.1) 
SNLI                              %            
     & 84.3 (0.2) & 66.9 (1.5)  & -1.3 \\   %& 79.5(0.1)
\bottomrule
\end{tabular}
    \caption{\label{tab:NLIablation}
    Results of the ablation study on auxiliary datasets using \bert on MNLI (the target task). 
    While the in-distribution performance is hardly affected when a specific auxiliary dataset is excluded,
    performance on the challenging data varies (difference shown in $\Delta$).
    }
\end{center}
%}
\end{table}

On \hans, MTL improves the accuracy significantly for \bert but not for \roberta.
To confirm the result, we additionally experimented with \robertal and obtained consistent results:
MTL achieves an accuracy of 75.7 (2.1) on \hans,
similar to the STL result, 77.1 (1.6).
One potential explanation is that RoBERTa is already sufficient for providing good generalization from minority examples in MNLI. 

In addition, both MTL and \roberta yiedls biggest improvement on \texttt{lexical overlap},
as shown in the results on \hans by category (\reftab{hans_category}),
We believe the reason is that \texttt{lexical overlap} is the most representative pattern among high-overlap and non-entailment training examples.
In fact, 
85\% of the 727 \hans-like examples belongs to \texttt{lexical overlap}.
This suggests that further improvement on \hans may require better data coverage on other categories.

On \paws, MTL consistently yields large improvement across pre-trained models.
Given that QQP has fewer minority examples resembling the patterns in \paws,
which is also harder to learn (\refsec{paws}),
the results show that MTL is an effective way to improve generalization when the minority examples are scarce.
Next, we investigate why MTL is helpful.


\begin{table}[t]
%\footnotesize{
\begin{center}
\begin{tabular}{lrrr}
\toprule
  Removed   &  \textbf{QQP} & \textbf{\pawsqqp} & $\Delta$ \\ 
 \midrule

None
     &  91.3 (.07) & 45.9 (2.1) & - \\  %& 90.4(0.1) 
\midrule
HANS           
      & 91.5 (.06) & 45.3 (1.8) & -0.6 \\   %& 90.3(0.3) 
MNLI                               %            
      & 91.2 (.11) & 42.3 (1.8) & -3.6 \\ %& 89.9(0.1) 
SNLI                              %            
     & 91.3 (.09) & 44.2 (1.3)  & -1.7 \\   %& 79.5(0.1)
\bottomrule
\end{tabular}
    \caption{\label{tab:PIablation}
    Results of the ablation study on auxiliary datasets using \bert on QQP (the target task). 
    While the in-distribution performance is hardly affected when a specific auxiliary dataset is excluded,
    performance on the challenging data varies (difference shown in $\Delta$). 
    }
\end{center}
%}
\end{table}

\paragraph{Improved generalization from minority examples.}
We are interested in finding how MTL helps generalization from minority examples.
One possible explanation is that the challenging data in the auxiliary datasets 
prevent the model from learning suprious patterns.
However, the ablation studies on auxiliary datasets in \reftab{NLIablation} and \reftab{PIablation}
show that the challenging datasets are not much more helpful than benchmark datasets.
The other possible explanation is that MTL reduces sample complexity for learning from the minority examples in the \emph{target dataset}.
To verify this, we remove minority examples from both the auxiliary and the target datasets,
and compare their effect on the robust accuracy.

We focus on PI because MTL shows largest improvement there.
In Table~\ref{tab:MTLablation}, we show the results after removing minority examples in the target dataset, QQP, and the auxiliary dataset, MNLI, respectively.
We also add a control baseline where the same amounts of randomly sampled examples are removed.
The results confirm our hypothesis:
without the minority examples in the target dataset,
MTL is only marginally better than STL on \pawsqqp.
In contrast, 
removing minority examples in the auxiliary dataset has a similar effect to removing random examples;
both do not cause significant performance drop.
Therefore, we conclude that MTL improves robust accuracy by improving generalization from minority examples in the target dataset.

\paragraph{Takeaway.}
These results suggest that
both pre-training and MTL do not enable extrapolation,
instead, they improve generalization from minority examples in the (target) training set.
Thus it is important to increase coverage of diverse patterns in the data to improve robustness to spurious correlations.







\begin{table}[ht]
\begin{center}
\begin{tabular}{lrrr}
\toprule
  Removed   &  \textbf{QQP} & \textbf{\pawsqqp} & $\Delta$ \\ 
 \midrule

None
     &  91.3 (.07) & 45.9 (2.1) & - \\  
\midrule

\multicolumn{4}{l}{\textit{random examples}} \\
QQP           
      & 91.3 (.03) & 44.3 (.31 ) &  -1.6\\    
MNLI                             %            
      & 91.4 (.02) & 45.0 (1.5 ) &  -0.9\\ 

\multicolumn{4}{l}{\textit{minority examples}} \\
QQP           
      & 91.3 (.09) & \textbf{38.2} (.73) & -7.7 \\    
MNLI                             %            
      & 91.3 (.08) & 44.3 (2.0) & -1.6 \\ 
\bottomrule
\end{tabular}
    \caption{\label{tab:MTLablation}
    Ablation study on the effect of minority examples in the auxiliary (MNLI) and the target (QQP) datasets in MTL with \bert.
    For MNLI, we removed 727 non-entailment examples with 100\% overlap.
    For QQP, we removed 228 non-paraphrase examples with 100\% overlap.
    We also removed equal amounts of random examples in the control experiments.
    We ran $t$-tests for the mean accuracies after minority removal and random removal based on five runs, and numbers with a significant difference ($p<0.001$) are bolded.
    The improvement from MTL mainly comes from better generalization from minority examples in the \emph{target dataset}.
    }
\end{center}
\end{table}



